Individual Calibration with Randomized Forecasting

Machine learning applications often require calibrated predictions, e.g. a 90\% credible interval should contain the true outcome 90\% of the times. However, typical definitions of calibration only require this to hold on average, and offer no guarantees on predictions made on individual samples. Thus, predictions can be systematically over or under confident on certain subgroups, leading to issues of fairness and potential vulnerabilities. We show that calibration for individual samples is possible in the regression setup if the predictions are randomized, i.e. outputting randomized credible intervals. Randomization removes systematic bias by trading off bias with variance. We design a training objective to enforce individual calibration and use it to train randomized regression functions. The resulting models are more calibrated for arbitrarily chosen subgroups of the data, and can achieve higher utility in decision making against adversaries that exploit miscalibrated predictions.

==> experiments.tex <==
% \section{Experiments}

% \subsection{Toy Data}

% \subsection{Fairness}

% We use the income dataset. We show that the classifier is always miscalibrated with respect to every feature. Even after we choose certain subgroups to recalibrate, the ones not selected are still miscalibrated. We show that with our method, every subgroup is calibrated. Not even an adversary can optimize for a subgroup where calibration fails. 

% We use two ways to find subgroups which may be miscalibrated. One of them is to choose several random combinations of (somewhat sensitive) features. This corresponds to making sure that pre-defined groups are well calibrated. The other one is to choose the worst cast miscalibrated set. Imagine that given the trained forecaster, some previously unidentified groups may, based on their  mistreatment by the forecaster, declare that they are a disadvantaged group. 

% \begin{figure}
%     \centering
%     % \includegraphics{}
%     \caption{Calibration of several potentially sensitive, but usually not considered attributes.}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure*}
% \centering 
% \begin{tabular}{c}
% \includegraphics[width=1.0\linewidth]{plots/calibration_plot_over.pdf} \\
% \includegraphics[width=1.0\linewidth]{plots/calibration_plot_under.pdf}
% \end{tabular}
% \caption{Calibration curve against worst-case adversary. The adversary has access to the test data and the learned forecaster, and finds the subset that is most under/over estimated.} 
% \end{figure*}
% \subsection{Exploration-Exploitation Trade-off}

% Consider the following 
